Designing a Direct Feedback Loop between Humans and Convolutional Neural Networks through Local Explanations

The local explanation provides heatmaps on images to explain how Convolutional Neural Networks (CNNs) derive their output. Due to its visual straightforwardness, the method has been one of the most popular explainable AI (XAI) methods for diagnosing CNNs. Through our formative study (S1), however, we captured ML engineers' ambivalent perspective about the local explanation as a valuable and indispensable envision in building CNNs versus the process that exhausts them due to the heuristic nature of detecting vulnerability. Moreover, steering the CNNs based on the vulnerability learned from the diagnosis seemed highly challenging. To mitigate the gap, we designed DeepFuse, the first interactive design that realizes the direct feedback loop between a user and CNNs in diagnosing and revising CNN's vulnerability using local explanations. DeepFuse helps CNN engineers to systemically search "unreasonable" local explanations and annotate the new boundaries for those identified as unreasonable in a labor-efficient manner. Next, it steers the model based on the given annotation such that the model doesn't introduce similar mistakes. We conducted a two-day study (S2) with 12 experienced CNN engineers. Using DeepFuse, participants made a more accurate and "reasonable" model than the current state-of-the-art. Also, participants found the way DeepFuse guides case-based reasoning can practically improve their current practice. We provide implications for design that explain how future HCI-driven design can move our practice forward to make XAI-driven insights more actionable.

==> sections/9999_ideation.tex <==
__________01_Intro__________
***DNN applied in an area where mistake can cause critical issue 
tumor diagnosis~\cite{zhen2020deep}

***Case-based reasoning
capturing expert knowledge on explanation methods~\cite{darias2022using}

*** why (contextual) bias can be detremental for model accuracy
"These biased models suffer from the poor generalization capability when evaluated on unbiased datasets - AND VICE VERSA"~\cite{lee2021learning}
data balance is important that represent social and demographic traits~\cite{goyal2022fairness}

__________02_RelatedWork__________

***survey paper
XAI tool survey and benchmarking~\cite{bodria2021benchmarking}
XAI design in the context of human factors, category of XAI and eval methods~\cite{mohseni2021multidisciplinary}
There are more comprehensive survey available for visual analytic tools designed for ML engineers~\cite{yuan2021survey}, visualization techniques for trustworthy ML models~\cite{chatzimparmpas2020state}

A survey of visual analytics tech~\cite{yuan2021survey}

review of taxonomy of XAI~\cite{speith2022review}

***hci+dnn inspection only
\textit{Prospector}~\cite{krause2016interacting}
\textit{Squares}~performance visualization for multiclass classifier~\cite{ren2016squares},
visual analytic approach that provides acyclic graph to understand CNNs~\cite{liu2016towards}
MLCube Explorer~\cite{kahng2016visual} provided model performance comparison serves, making model performance evaluation and model selection processes more straightforward.
\text{ActiVis} DNN model explorator~\cite{kahng2017cti}
Understanding the CNN's characteristics in multiclass problem~\cite{bilal2017convolutional}
inspecting RNN for NLP tasks~\cite{ming2017understanding}
provide rule-based knowledge representation using RuleMatrix~\cite{ming2018rulematrix}
GAMUT-design probe that helps how data scientists undrstand ML models~\cite{hohman2019gamut}
SUMMIT: Helping people to understand a ``big picture'' behind DNN by leveraging summarizing techniques ~\cite{hohman2019s}
CNN explore~\cite{wang2020cnn}
ExplainExplorer~\cite{collaris2020explainexplore}
DeepEyes apply non-linear dimensionality-reduction techniques, helping people to better understand how classes are defined through visual analytic system~\cite{pezzotti2019dimensionality}
The What-if tool~\cite{wexler2019if}
Dodrio: understanding transformer models~\cite{wang2021dodrio}
NeuroCartography~\cite{park2021neurocartography}

***general visual analytics method 
multi-class classifier diagnosis~\cite{alsallakh2014visual}

***explanation + steer
one of the early work: providing the way to mix multiple classifiers~\cite{talbot2009ensemblematrix}
ModelTracker~\cite{amershi2015modeltracker} provided model performance comparison serves
Tenserflow Graph Visualizer~\cite{wongsuphasawat2017visualizing} show the hierarchical structure annotated in the source code for DNN dev.
Combine multiple XAI techniques in model diagnosis and refinement explAIner~\cite{spinner2019explainer}

***Contextual bias
men also like shopping~\cite{zhao2017men}
Balendced datasets are not enough~\cite{wang2019balanced}
Women also snowboard~\cite{hendricks2018women}
don't judge object by its context~\cite{singh2020don}
overparameterization can result in worsening ``spurious correlation''~\cite{sagawa2020investigation}
Finding small sampled groups when applying model pruning~\cite{hooker2020characterising}
gender bias in VQA - distribution of answers differe between men and women~\cite{hirota2022gender}

***ML computational approach for XAI + steer
rule-driven steering~\cite{hu2016harnessing}
include feature attribution into obj function to incorporate prior in model building~\cite{liu2019incorporating}
Human prior reasoning design, DAFT~\cite{kim2019learning}
VRX helps interpreting the nn using "structural visual concept"~\cite{ge2021peek}

***model attention direct adjustment
ABN~\cite{fukui2019attention}
Direct editing of attention map~\cite{mitsuhara2019embedding}
GNES Graph NN~\cite{gao2021gnes}
GRADIA~\cite{gao2022aligning}
RES~\cite{gao2022res}

__________04_DEEPFUSE__________
***design motivation for deepfuse
-. apply croudsourcing to find features in image classifier to attain global interpretability: what do you mean~\cite{balayn2021you}
-. Reasonability matrix~\cite{gao2022aligning}
***fairness in vis
helping people to determine uinderrerpesented subgroup - bias+hci~\cite{cabrera2019fairvis}
"toolkit designers should empirically study how practitioners apply
fairness toolkits to more complex tasks with a wider range of datasets"~\cite{deng2022exploring}

__________06_IMP__________
***detecting adversarial
Inspecting vulnerabilities of adversarial attack through visual analytics~\cite{ma2019explaining}
Bluff ~\cite{das2020bluff}
UnMask for adversarial detection and defense~\cite{freitas2020unmask}
SkeletonVis~\cite{park2021skeletonvis}


*** generalizability (different tasks, different datasets)
How we can help ml engineers to use fairness toolkit?~\cite{deng2022exploring}
"toolkit designers should empirically study how practitioners apply
fairness toolkits to more complex tasks with a wider range of datasets"~\cite{deng2022exploring}

***importance of providing the right balance of human involvement
***Effectiveness of human-guided model training AutoML


***some interesting trade-offs

1. model interpretability (black box vs white) - accuracy relationship
"One side postulates that model accuracy and explainability are inversely related, leading practitioners to use black-box models when high accuracy is important. The other side of this argument holds that the accuracy-explainability trade-off is rarely observed in practice and consequently, that simpler interpretable models should always be preferred. ...
In summary, contrary to both positions in the literature, we neither observed a direct trade-off between accuracy and explainability nor found interpretable models to be superior in terms of explainability"~\cite{bell2022s}
2. degree of human involvement - accuracy relationship
"On synthetic and real data we illustrate how “arguing” with a deep model about its explanations can actually help to revise the model, if it is right for the wrong reasons"~\cite{shao2020towards}
***how human's reasoning thought to be right can result in accurate prediction? - more case-based studies needed.
~\cite{abdul2020cogam}
human-guided machine learning using AutoML~\cite{gil2019towards}
Visus~\cite{santos2019visus}
Importance of embedding domain knowledge~\cite{collaris2020explainexplore} 
3. degree of humans' reasonableness - accuracy relationship


***Data iteration
"ML practitioners reveal that they improve model performance frequently by iterating on their data"~\cite{hohman2020understanding}
CHAMELEON lets users compare data features, training/testing splits, and performance across data versions~\cite{hohman2020understanding}

***evaluation metric
for ai novice, usefulness and satisfaction human-ai performance is priority. for the ai experts, the importance shifts toward model trustworthiness and fidelity of explanation for model debugging.~\cite{mohseni2021multidisciplinary}


etc
***general good words
ML forgetting issue~\cite{kirkpatrick2017overcoming}




